Bounded support in linear random coefficient models: Identification and variable selection

We consider linear random coefficient regression models, where the regressors are allowed to have a finite support. First, we investigate identifiability, and show that the means and the variances and covariances of the random coefficients are identified from the first two conditional moments of the response given the covariates if the support of the covariates, excluding the intercept, contains a Cartesian product with at least three points in each coordinate. We also discuss ientification of higher-order mixed moments, as well as partial identification in the presence of a binary regressor. Next we show the variable selection consistency of the adaptive LASSO for the variances and covariances of the random coefficients in finite and moderately high dimensions. This implies that the estimated covariance matrix will actually be positive semidefinite and hence a valid covariance matrix, in contrast to the estimate arising from a simple least squares fit. We illustrate the proposed method in a simulation study.

==> asymptotic_first_moments.tex <==

We need some assumptions to prove asymptotic results for the LASSO and his adaptive version in the linear regression model \eqref{random:coefficient:model:first:moments} of the first moments.

\begin{assumption} \label{ass:moments:first:moments} %\hfill\\
	We assume that
	\begin{enumerate}[label=\normalfont{(A\arabic*)},leftmargin=9.9mm]
		\item the random coefficients $\f{A}$ have finite second moments, \label{moments:first:moments:B1}
		\item the covariates $\f{X}=(1,\f{W^\top})^\top$ (or rather $\f{W}$) have finite forth moments, \label{moments:first:moments:B2}
		\item the symmetric second moment matrix 
		\begin{align*} 
		\mathrm{C}^{\mu} \defeq \E \big[\f{X}\,\f{X^\top}\big] \quad \in \R^{p \times p}
		\end{align*}
		of the covariates is positive definite. \label{moments:first:moments:B3}
		\setcounter{temp1}{\value{enumi}}
	\end{enumerate}
\end{assumption}

The last assumption is connected to the identification of the first moments, discussed in Proposition \ref{prop:onlyvariances}. The corresponding proof is provided in the supplement, Section \ref{sec:connection:identification:estimation}.

\begin{lemma} \label{lemma:Cmu:positive:definite}%\hfill\\
If the support of $\bW$ contains $p$ points $\f{w_1}, \dotsc, \f{w_p} \in \R^{p-1}$ in general position, then $\mathrm{C}^{\mu}$ is positive definite.
\end{lemma}
%
%\begin{proof} %\hfill\\
%Cf. Section \ref{sec:fixedp:proofs:first:moments}.
%\end{proof}


%Now we can give sufficient conditions for the sign-consistency of the LASSO. The proof is deferred to Section \ref{sec:fixedp:proofs:main:steps}.
%
%\begin{theorem} \label{theorem:LASSO:first:moments} %\hfill\\
%	Consider the linear regression model \eqref{random:coefficient:model:first:moments} and let Assumption \ref{ass:moments:first:moments} as well as the mutual incoherence condition
%	\begin{align}
%	\normiM{ \mathrm{C}_{S_\mu^c S_\mu}^{\mu} \, \big(\mathrm{C}_{S_\mu S_\mu}^{\mu}\big)^{-1} } < 1 \label{mutual:incoherence:first:moments}
%	\end{align}
%	%with $\mathrm{C}_{S_\mu^c S_\mu}^{\mu} \in \R^{(p-s_\mu) \times s_\mu}$ and $\big(\mathrm{C}_{S_\mu S_\mu}^{\mu}\big)^{-1} \in \R^{s_\mu \times s_\mu}$ 
%	be satisfied. If in addition $\lambda_n^{\mu} \to 0$ and $\sqrt{n} \, \lambda_n^{\mu} \to \infty$ hold, the LASSO $\widehat{\mu}_n^{\,\LA}$ as a solution to \eqref{def:LASSO:first:moments} is sign-consistent, 
%	\begin{align*}
%	\mathbb{P}\Big( \sign\big(\widehat{\mu}_n^{\,\LA}\big) = \sign\big(\mu^*\big)\Big) \to 1 \, , %\label{sign:consistency:LASSO:first:moments}
%	\end{align*}
%	and has estimation rate $\lambda_n^{\mu}$ on the support, 
%	\begin{align*}
%	\frac{1}{\lambda_n^{\mu}} \big( \widehat{\mu}_{n,S_\mu}^{\,\LA} - \mu_{S_\mu}^* \big) = \Op{1} \, . %\label{estimation:rate:LASSO:first:moments}
%	\end{align*} 
%\end{theorem}            
%
%\begin{proof} %\hfill\\
%	Cf. Section \ref{sec:fixedp:proofs:first:moments}.
%\end{proof}


%\begin{remark} \label{remark:disadvantage:LASSO}%\hfill\\
%	The mutual incoherence condition \eqref{mutual:incoherence:first:moments} is crucial for the sign-consistency of the LASSO, cf. \citet{Zou2006} and \citet{Wainwright2009}. The assumption can be dropped if an adaptive version is used. Moreover, the adaptive LASSO enjoys under homoscedasticity the oracle properties, cf. \citet{Zou2006}. That implies the selection of the true model by the estimator and an optimal estimation rate of $1/\sqrt{n}$. Theorem \ref{theorem:LASSO:first:moments} shows that the LASSO satisfies only one of these properties since the regularization parameter $\lambda_n^{\mu}$ tends slower to zero than the square root of the number $n$ of observations to infinity. 
%	%However, the adaptive LASSO enjoys these characteristics under heteroscedasticity, cf. \citet{Wagener2012}.
%\end{remark}


%\begin{remark} \label{remark:estimation:rate:least:squares:first:moments:1} %\hfill\\
%	For the sign-consistency and asymptotic normality of the adaptive LASSO also assumptions for the regularization parameter $\lambda_n^{\mu}$ are necessary. However, they depend on the estimation rate of the initial estimator. In the following we want to use the Least Squares Estimator for this purpose and hence we have to investigate its rate. The results in Section \ref{sec:fixedp:proofs:main:steps} lead to 
%	\begin{align}
%		\sqrt{n} \, \big( \widehat{\mu}_n^{\,\LS} - \mu^* \big) = \Op{1} \,, \label{estimation:rate:least:squares:first:moments}
%	\end{align} 
%	provided that Assumption \ref{ass:moments:first:moments} is satisfied, see Remark \ref{remark:estimation:rate:least:squares:first:moments:2} for more details.
%\end{remark}


Now we can consider in the subsequent theorem the sign-consistency and asymptotic normality of the adaptive LASSO on the true support $S_{\mu}$. For this purpose we define the positive semi-definite matrix
\begin{align}
\mathrm{B}^{\mu} \defeq \E \Big[ \big(\f{X^\top} \Sigma^* \, \f{X}\big) \, \f{X}\,\f{X^\top} \Big] \quad \in \R^{p \times p}\,. \label{def:B:first:moments}
\end{align}
The proof is deferred to Section \ref{sec:fixedp:proofs:main:steps} as well.

\begin{theorem} \label{theorem:adaptive:LASSO:first:moments} %\hfill\\
	Consider the linear regression model \eqref{random:coefficient:model:first:moments} and let Assumption \ref{ass:moments:first:moments} be satisfied. If in addition $\lambda_n^{\mu} \to 0$, $\sqrt{n} \, \lambda_n^{\mu} \to 0$ and $n \, \lambda_n^{\mu} \to \infty$ hold, the adaptive LASSO $\widehat{\mu}_n^{\,\AL}$, as a solution to \eqref{def:adaptive:LASSO:first:moments} with initial estimator $\widehat{\mu}_n^{\,\init}$ that satisfies $\sqrt{n} \, \big( \widehat{\mu}_{n}^{\,\init} - \mu^* \big) = \Op{1}$, is sign-consistent, 
	\begin{align}
	\mathbb{P}\Big( \sign\big(\widehat{\mu}_n^{\,\AL}\big) = \sign\big(\mu^*\big)\Big) \to 1 \, , \label{sign:consistency:adaptive:LASSO:first:moments}
	\end{align}
	and satisfies the asymptotic normality
	\begin{align}
	\sqrt{n} \, \big( \widehat{\mu}_{n,S_{\mu}}^{\,\AL} - \mu_{S_\mu}^* \big) ~ \stackrel{d} \longrightarrow ~ \mathcal{N}_{s_{\mu}} \Big( \f{0}_{s_{\mu}} ,\big(\mathrm{C}_{S_\mu S_\mu}^{\mu}\big)^{-1} \, \mathrm{B}_{S_{\mu} S_{\mu}}^{\mu} \, \big(\mathrm{C}_{S_\mu S_\mu}^{\mu}\big)^{-1} \Big) \, . \label{asymptotic:normality:adaptive:LASSO:first:moments}
	\end{align} 
\end{theorem}            
%
%\begin{proof} %\hfill\\
%	Cf. Section \ref{sec:fixedp:proofs:first:moments}.
%\end{proof}      

\begin{remark} \label{remark:limiting:matrix:first:moments} %\hfill\\
	Similar to Remark \ref{remark:limiting:matrix:second:moments} we obtain under Assumption \ref{moments:first:moments:B1} and \ref{moments:first:moments:B2} the expected values
	
	%The rescaled gram matrices can also be written by
	%\begin{align*}
	%	\frac{1}{n} \, \big(\Xmu\big)^\top \Xmu = \frac{1}{n} \sum_{i=1}^n \f{X_i}\,\f{X_i^\top} \,.
	%\end{align*}
	%Hence the matrix is also called the sample second moment matrix. 
	
	\begin{align*}
		\E \bigg[ \frac{1}{n} \, \big(\Xmu\big)^\top \Xmu \bigg]  = \mathrm{C}^{\mu}\,,\quad  \E \bigg[ \frac{1}{n} \, \big(\Xmu\big)^\top \Omega_n^{\mu} \, \Xmu \bigg] = \mathrm{B}^{\mu}  %\label{mean:matrix:B:first:moments}
	\end{align*}
	and the almost sure convergences 
	\begin{align*}
		\normiM{ \frac{1}{n} \, \big(\Xmu\big)^\top \Xmu - \mathrm{C}^{\mu}} ~ \stackrel{a.s.} \longrightarrow~ 0 \,, \quad \normiM{ \frac{1}{n} \, \big(\Xmu\big)^\top \Omega_n^{\mu} \, \Xmu - \mathrm{B}^{\mu}} ~ \stackrel{a.s.} \longrightarrow~ 0 \,, %\label{limiting:matrix:C:first:moments}
	\end{align*}
	where the second moment matrix $\mathrm{C}^{\mu}$ of $\f{X}$ is given in \ref{moments:first:moments:B3}, the conditional covariance matrix $\Omega_n^{\mu}$ in \eqref{cov:epsilon:first:moments} and $\mathrm{B}^{\mu}$ in \eqref{def:B:first:moments}.
\end{remark}

In the subsequent lemma we formulate the analog result for the rescaled gradient of the empirical quadratic loss function for the first moments.

\begin{lemma} \label{lemma:gradient:bounded:first:moments} %\hfill\\
	Suppose that Assumption \ref{moments:first:moments:B1} holds. Then the random vectors 
	\begin{align*}
		Z_n^{\mu} = -\frac{\sqrt{n}}{2} \,  \nabla \loss_{\mu,n}^{\, \LS} \big(\mu^*\big) = \frac{1}{\sqrt{n}} \, \big(\Xmu\big)^\top \epsmu 
	\end{align*} 
	satisfy 
	\begin{align*}
		\E\big[ Z_n^{\mu} \, \big| \, \Xmu \big] &= \f{0}_p \quad \text{and} \quad \cov\big( Z_n^{\mu} \, \big| \, \Xmu \big) = \frac{1}{n}\, \big(\Xmu\big)^\top \Omega_n^{\mu} \, \Xmu \,  .
	\end{align*}
	If in addition Assumption \ref{moments:first:moments:B2} holds, then
	\begin{align*}
		\cov\big( Z_n^{\mu} \big) = \mathrm{B}^{\mu} \,, %\label{convergence:covariance:gradient:first:moments}
	\end{align*}
	which implies
	\begin{align*}
		Z_n^{\mu} = \Op{1} \, .
	\end{align*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:gradient:bounded:first:moments}] %\hfill\\
	Similar to the proof of Lemma \ref{lemma:gradient:bounded:second:moments:1}. In doing so we use the results in Remark \ref{remark:limiting:matrix:first:moments}.
\end{proof}            


\begin{proof}[Proof of Theorem \ref{theorem:adaptive:LASSO:first:moments}] %\hfill\\
	Similar to the proof of Theorem \ref{theorem:adaptive:LASSO:second:moments}. Note that we obtain especially
	\begin{align}
		\normiM{\bigg(\frac{1}{n} \, \big(\Xmu\big)^\top  \Xmu \bigg)^{-1} - \big(\mathrm{C}^{\mu} \big)^{-1} } ~ \stackrel{a.s.} \longrightarrow ~ 0  \label{proof:theorem:LASSO:first:moments:1} 
	\end{align}
	and
	\begin{align}
		\sqrt{n} \, \big( \widehat{\mu}_{n,S_{\mu}}^{\,\AL} -  \mu_{S_\mu}^* \big) = \bigg(\frac{1}{n} \, \big(\XmuS\big)^\top  \XmuS \bigg)^{-1} \frac{1}{\sqrt{n}} \, \big(\XmuS\big)^\top \epsmu  + \op{1} \label{proof:theorem:adaptive:LASSO:first:moments:3} 
	\end{align}
	which is crucial for the proof of Lemma \ref{lemma:gradient:bounded:second:moments:2}.
\end{proof}   



==> asymptotic_second_moments.tex <==
% 
%In the following we provide analog results as in Theorem \ref{theorem:adaptive:LASSO:first:moments} in Section \ref{sec:fixedp:first:moments} for the half-vectorization $\sigma^*$ of the covariance matrix $\Sigma^*$ of the random coefficients $\f{A}$. Note that the linear regression model \eqref{random:coefficient:model:second:moments} depends on the estimator $\widehat{\mu}_n$ for the first moments $\mu^*$. For this purpose we choose throughout this section the adaptive LASSO $\widehat{\mu}_n^{\,\AL}$, which is defined in \eqref{def:adaptive:LASSO:first:moments}, with the Least Squares Estimator $ \widehat{\mu}_n^{\,\LS}$ as initial estimator. Once again we need some assumptions for the these results.
%

%
%\begin{remark}
%The matrix 
%\begin{align*}
%\E \Big[ (1,2\,\f{W^\top})^\top\,(1,2\,\f{W^\top})\Big] \quad \in \R^{p \times p}
%\end{align*}
%is a submatrix of $\mathrm{C}^{\sigma}$ because of the definition \eqref{def:v} of the vector transformation $\ov(\,\cdot\,)$. If Assumption \ref{moments:second:moments:B3} is satisfied, then also the above submatrix has to be positive definite. This implies the positive definiteness of $\mathrm{C}^{\mu}= \E [\f{X}\,\f{X^\top}]$ as well. Hence, if Assumption \ref{ass:moments:second:moments} holds, also Assumption \ref{ass:moments:first:moments} is satisfied.
%\end{remark}
%
%Furthermore, Assumption \ref{moments:second:moments:B3} is connected to the identification of the first and second moments discussed in Theorem \ref{prop:necsuffcond}. 

%Now we give sufficient conditions, similar to Theorem \ref{theorem:LASSO:first:moments}, for the sign-consistency of the LASSO. The proof is deferred to Section \ref{sec:fixedp:proofs:main:steps}.
%
%\begin{theorem} \label{theorem:LASSO:second:moments} %\hfill\\
%	Consider the linear regression model \eqref{random:coefficient:model:second:moments} with $\widehat{\mu}_n = \widehat{\mu}_n^{\, \AL}$ and let Assumption \ref{ass:moments:second:moments} as well as the mutual incoherence condition
%	\begin{align}
%		\normiM{ \mathrm{C}_{S_\sigma^c S_\sigma}^{\sigma} \, \big(\mathrm{C}_{S_\sigma S_\sigma}^{\sigma}\big)^{-1} } < 1 \label{mutual:incoherence:second:moments}
%	\end{align}
%	%with $\mathrm{C}_{S_\sigma^c S_\sigma}^{\sigma} \in \R^{(p-s_\sigma) \times s_\sigma}$ and $\big(\mathrm{C}_{S_\sigma S_\sigma}^{\sigma}\big)^{-1} \in \R^{s_\sigma \times s_\sigma}$ 
%	be satisfied. If in addition $\lambda_n^{\mu} \to 0$, $\sqrt{n} \, \lambda_n^{\mu} \to \infty$, $n \, \lambda_n^{\mu} \to \infty$ and $\lambda_n^{\sigma} \to 0$, $\sqrt{n} \, \lambda_n^{\sigma} \to \infty$ hold, the LASSO $\widehat{\sigma}_n^{\,\LA}$ as a solution to \eqref{def:LASSO:second:moments} is sign-consistent, 
%	\begin{align*}
%		\mathbb{P}\Big( \sign\big(\widehat{\sigma}_n^{\,\LA}\big) = \sign\big(\sigma^*\big)\Big) \to 1 \, , %\label{sign:consistency:LASSO:second:moments}
%	\end{align*}
%	and has estimation rate $\lambda_n^{\sigma}$ on the support, 
%	\begin{align*}
%		\frac{1}{\lambda_n^{\sigma}} \big( \widehat{\sigma}_{n,S_\sigma}^{\,\LA} - \sigma_{S_\sigma}^* \big) = \Op{1} \, . %\label{estimation:rate:LASSO:second:moments}
%	\end{align*} 
%\end{theorem} 
%
%For the disadvantages of the Lasso in comparison to his adaptive version see the discussion in Remark \ref{remark:disadvantage:LASSO}. Moreover, the results in Section \ref{sec:fixedp:proofs:main:steps} lead again to an optimal estimation rate of the Least Squares Estimator,
%\begin{align}
%\sqrt{n} \, \big( \widehat{\sigma}_n^{\,\LS} - \sigma^* \big) = \Op{1} \,, \label{estimation:rate:least:squares:second:moments}
%\end{align} 
%provided that Assumption \ref{ass:moments:second:moments} is satisfied, see Remark \ref{remark:estimation:rate:least:squares:second:moments} for more details.\\

%In the subsequent theorem we provide, similar to Theorem \ref{theorem:adaptive:LASSO:first:moments}, a statement about the sign-consistency of the adaptive LASSO for the second central moments and give a normality result on the true support $S_{\sigma}$. For this purpose we define the positive semi-definite matrix
%where $\Psi^*$ is given in \eqref{def:psi} and contains the fourth central moments of the coefficients $\f{A}$. The proof is deferred to Section \ref{sec:fixedp:proofs:main:steps} as well. 
%
%
%\begin{theorem} \label{theorem:adaptive:LASSO:second:moments} %\hfill\\
%	Consider the linear regression model \eqref{random:coefficient:model:second:moments} with $\widehat{\mu}_n = \widehat{\mu}_n^{\, \AL}$, where $\widehat{\mu}_n^{\, \AL}$ is a solution to \eqref{def:adaptive:LASSO:first:moments} with initial estimator $\widehat{\mu}_n^{\,\init}$ that satisfies $\sqrt{n} \, \big( \widehat{\mu}_{n}^{\,\init} - \mu^* \big) = \Op{1}$ and regularization parameter $\lambda_n^{\mu}$ that satisfies $\lambda_n^{\mu} \to 0$, $\sqrt{n} \, \lambda_n^{\mu} \to 0$ and $n \, \lambda_n^{\mu} \to \infty$. Moreover, let Assumption \ref{ass:moments:second:moments} be satisfied. If in addition $\lambda_n^{\sigma} \to 0$, $\sqrt{n} \, \lambda_n^{\sigma} \to 0$, $n \, \lambda_n^{\sigma} \to \infty$ hold, the adaptive LASSO $\widehat{\sigma}_n^{\,\AL}$, as a solution to \eqref{def:adaptive:LASSO:second:moments} with initial estimator $\widehat{\sigma}_n^{\,\init}$ that satisfies $\sqrt{n} \, \big( \widehat{\sigma}_{n}^{\,\init} - \sigma^* \big) = \Op{1}$, is sign-consistent, 
%	\begin{align}
%		\mathbb{P}\Big( \sign\big(\widehat{\sigma}_n^{\,\AL}\big) = \sign\big(\sigma^*\big)\Big) \to 1 \, , \label{sign:consistency:adaptive:LASSO:second:moments}
%	\end{align}
%	and satisfies the asymptotic normality
%	\begin{align}
%		\sqrt{n} \, \big( \widehat{\sigma}_{n,S_{\sigma}}^{\,\AL} - \sigma_{S_\sigma}^* \big) ~ \stackrel{d} \longrightarrow ~ \mathcal{N}_{s_{\sigma}} \Big( \f{0}_{s_{\sigma}} ,\big(\mathrm{C}_{S_\sigma S_\sigma}^{\sigma}\big)^{-1} \, \mathrm{B}_{S_{\sigma} S_{\sigma}}^{\sigma} \, \big(\mathrm{C}_{S_\sigma S_\sigma}^{\sigma}\big)^{-1} \Big) \, . \label{asymptotic:normality:adaptive:LASSO:second:moments}
%	\end{align} 
%\end{theorem}            
%%
%\begin{proof} %\hfill\\
%	Cf. Section \ref{sec:fixedp:proofs:second:moments}.
%\end{proof}      


%\begin{remark} %\hfill\\
%The results in Section \ref{sec:fixedp:proofs:main:steps} show that the asymptotic normality of the the adaptive Lasso $\widehat{\sigma}_{n}^{\,\AL}$ on the true support $S_{\sigma}$ is independent of the fact whether we know the first moments in advance or whether we estimate them simultaneously with an appropriate estimator. See Remark \ref{remark:adaptive:LASSO:second:moments} for more details. 
%
%The asymptotic covariance matrix in \eqref{asymptotic:normality:adaptive:LASSO:second:moments} can be degenerate since we have no further assumption on $\mathrm{B}^{\mu}$. If $\mathrm{B}_{S_{\sigma} S_{\sigma}}^{\sigma}$ is positive definite then the asymptotic covariance of the rescaled estimation error of the adaptive LASSO is positive definite as well.
%
%Moreover, by Remark \ref{remark:adaptive:LASSO:second:moments} in Section  \ref{sec:fixedp:proofs:main:steps} it follows that the Least Squares Estimator, given by
%\begin{align}
%	\widehat{\sigma}_n^{\,\LS} \in \rho_{\sigma,n}^{\,\LS} \defeq  \underset{\beta \in \R^{\frac{p(p+1)}{2}}}{\arg\min} ~ \loss_{\sigma,n}^{\, \LS} \big(\beta\big) \,, \label{def:ls:second:moments}
%\end{align}
%satisfies
%\begin{align*}
%	\sqrt{n} \, \big( \widehat{\sigma}_n^{\,\LS} - \sigma^* \big) \longrightarrow ~ \mathcal{N}_{\frac{p(p+1)}{2}} \Big( \f{0}_{\frac{p(p+1)}{2}} ,\big(\mathrm{C}^{\sigma}\big)^{-1} \, \mathrm{B}^{\sigma} \, \big(\mathrm{C}^{\sigma}\big)^{-1} \Big) \,.
%\end{align*}
%Hence it can be used as initial estimator in Theorem \ref{theorem:adaptive:LASSO:second:moments}. Also the ordinary LASSO, given by
%\begin{align*}
%	\widehat{\sigma}_n^{\,\LA} \in \rho_{\sigma,n,\lambda_n^{\sigma}}^{\,\LA} &\defeq \underset{\beta \in \R^{\frac{p(p+1)}{2}}}{\arg\min} ~ \bigg( \loss_{\sigma,n}^{\, \LS} \big(\beta\big) + 2 \lambda_n^{\sigma}  \norme{\beta} \bigg)  %\label{def:LASSO:second:moments}
%\end{align*} 
%with regularization parameter $\lambda_n^{\sigma}>0$, or the Ridge Estimator,
%\begin{align*}
%	\widehat{\sigma}_n^{\,\Rid} \in \rho_{\sigma,n,\lambda_n^{\sigma}}^{\,\Rid} &\defeq \underset{\beta \in \R^{\frac{p(p+1)}{2}}}{\arg\min} ~ \bigg( \loss_{\sigma,n}^{\, \LS} \big(\beta\big) + 2 \lambda_n^{\sigma}  \normzq{\beta} \bigg)  
%\end{align*}
%are a potential choices, see \citet[Theorem 2]{Knight2000}.





%\end{remark}



==> simulation_RCM_fixed_p.tex <==

 We consider the linear random coefficient regression model \eqref{random:coefficient:model:intercept}  with normally distributed random coefficients $\f{A} = \big( B_0,B_1,\dotsc,B_5 \big)^\top \sim \mathcal{N}_6 \big(\mu^*,\Sigma^*\big)$ with mean vector $\mu^* = \big( 40,15,0,-10,20,0 \big)^\top$ and covariance matrix
\begin{align*}
\Sigma^* = \begin{bmatrix}   
10 & 15.65 & -5.20 & 0 & 0 & 0\\
15.65 & 50 & 0 & 12.65 & 0 & 0\\
-5.20 & 0 & 30 & -12.25 & 0 & 0\\
0 & 12.65 & -12.25 & 20 & 0 & 0\\
0 & 0 &  0 & 0 & 0 & 0 \\
0 & 0 &  0 & 0 & 0 & 0      
\end{bmatrix} \,.
\end{align*} 
The exact correlation coefficients are $\rho_{12} = 0.7$, $\rho_{13} = -0.3$, $\rho_{24} = 0.4$, $\rho_{34} = -0.5$ and evidently $\rho_{14} = \rho_{23} = 0$.
Furthermore, the covariates are $ W_1,\dotsc,W_5$ are assumed to be independent and identically distributed. We simulate $n$ pairs $(Y_1,\f{W_1^\top})^\top,\dotsc,(Y_n,\f{W_n^\top})^\top$ of data according to this model and use them for variable selection and estimation of the moments of the random coefficients $\f{A}$ with the adaptive LASSO. The appropriate estimators $\widehat{\mu}_n^{\,\AL}$ and $\widehat{\sigma}_n^{\,\AL}$ with regularization parameters $\lambda_n^{\mu}, \lambda_n^{\sigma}>0$ are given in \eqref{def:adaptive:LASSO:first:moments} and \eqref{def:adaptive:LASSO:second:moments}. The initial estimator is always the  Least Squares Estimator, see \eqref{def:ls:second:moments} (for the first moments the empirical quadratic loss function is $\loss_{\mu,n}^{\, \LS}$). Moreover, note that the mean and variance of the random intercept $B_0$ are not penalized in our simulation with the function \texttt{glmnet()}. This is plausible since it includes the deterministic intercept as well as a random error which is not affected by the covariates.

In each of the following scenarios we conduct two Monte Carlo simulations with $m=10.000$ iterations each to illustrate the sign-consistency and asymptotic normality of $\widehat{\mu}_n^{\,\AL}$ and $\widehat{\sigma}_n^{\,\AL}$ in Theorem \ref{theorem:adaptive:LASSO:first:moments} and \ref{theorem:adaptive:LASSO:second:moments} for various sample sizes. In Simulation 1 we consider always $n_1=10.000$ and in the second one $n_2=100.000$. The regularization parameters are chosen such that there is a satisfactory trade-off between a high sign-recovery rate and a small estimation error. For this purpose we use $1000$ independent repetitions, run through a grid for $\lambda$ in each data set and determine the regularization parameters with correct number of degrees of freedom and the one with the smallest $\ell_2$ norm of the respective estimator error among these. Based on this information we choose the parameters in the Monte Carlo Simulation.  

\begin{itemize}
\item[(a)] \textbf{$\boldsymbol{\mathcal{U}[-1,1]}$ distributed covariates.} \\
We consider $W_1,\dotsc,W_5 \sim \mathcal{U}[-1,1]$ and the regularization parameters are given by $\lambda_{n_1}^{\mu}=0.4 , \lambda_{n_2}^{\mu}=0.2, \lambda_{n_1}^{\sigma}=16.5$ and $\lambda_{n_2}^{\sigma}=12.0$. For the sign-consistency we obtain
\begin{gather*}
	\mathbb{P}\Big( \sign\big(\widehat{\mu}_{n_1}^{\,\AL}\big) = \sign\big(\mu^*\big)\Big) = 0.9427\,,\qquad \mathbb{P}\Big( \sign\big(\widehat{\mu}_{n_2}^{\,\AL}\big) = \sign\big(\mu^*\big)\Big) = 0.9641 \,,\\
	\mathbb{P}\Big( \sign\big(\widehat{\sigma}_{n_1}^{\,\AL}\big) = \sign\big(\sigma^*\big)\Big) = 0.7513\,,\qquad \mathbb{P}\Big( \sign\big(\widehat{\sigma}_{n_2}^{\,\AL}\big) = \sign\big(\sigma^*\big)\Big) = 0.9127\,.
\end{gather*}
A comparison of the empirical and asymptotic densities of the rescaled estimation errors of the means and variances, which are unequal to zero, are shown in the following figures. Especially for the second moments the larger sample size increases the sign-recovery rate and also the empirical densities lie closer to the asymptotic ones.  \\

\begin{figure}[!h]       
	\centering
	\includegraphics[width=0.85\linewidth]{mu_unif[-1,1].eps}
	\caption{comparison of the densities of the rescaled estimation error of the means with $\mathcal{U}[-1,1]$ distributed covariates.}
\end{figure}

\hfill
\newpage

\begin{figure}[!h]       
	\centering	
	\includegraphics[width=0.85\linewidth]{sigma_unif[-1,1].eps}
	\caption{comparison of the densities of the rescaled estimation error of the variances with $\mathcal{U}[-1,1]$ distributed covariates.}
\end{figure}


\hfill
\newpage

\item[(b)] \textbf{$\boldsymbol{\mathcal{U}\{-1,0,1\}}$ distributed covariates.} \\
We consider $W_1,\dotsc,W_5 \sim \mathcal{U}\{-1,0,1\}$ uniform distributed on the set $\{-1,0,1\}$ and the regularization parameters are given by $\lambda_{n_1}^{\mu}=0.5 , \lambda_{n_2}^{\mu}=0.3, \lambda_{n_1}^{\sigma}=23.8$ and $\lambda_{n_2}^{\sigma}=17.4$. The following results are very similar to scenario (a), which confirms that three support points for each covariate are sufficient for the estimation of the first and second moments.

\begin{gather*}
	\mathbb{P}\Big( \sign\big(\widehat{\mu}_{n_1}^{\,\AL}\big) = \sign\big(\mu^*\big)\Big) = 0.9398\,,\qquad \mathbb{P}\Big( \sign\big(\widehat{\mu}_{n_2}^{\,\AL}\big) = \sign\big(\mu^*\big)\Big) = 0.9688 \,,\\
	\mathbb{P}\Big( \sign\big(\widehat{\sigma}_{n_1}^{\,\AL}\big) = \sign\big(\sigma^*\big)\Big) = 0.7045\,,\qquad \mathbb{P}\Big( \sign\big(\widehat{\sigma}_{n_2}^{\,\AL}\big) = \sign\big(\sigma^*\big)\Big) = 0.898\,.
\end{gather*}

\begin{figure}[h!]       
	\centering
	\includegraphics[width=0.85\linewidth]{mu_unif{-1,0,1}.eps}
	\caption{comparison of the densities of the rescaled estimation error of the means with $\mathcal{U}\{-1,0,1\}$ distributed covariates.}
\end{figure}

\hfill
\newpage

\begin{figure}[h!]       
	\centering
	\includegraphics[width=0.85\linewidth]{sigma_unif{-1,0,1}.eps}
	\caption{comparison of the densities of the rescaled estimation error of the variances with $\mathcal{U}\{-1,0,1\}$ distributed covariates.}
\end{figure}

\hfill
\newpage

\item[(c)] \textbf{$\boldsymbol{\mathcal{U}[0,1]}$ distributed covariates.} \\
We consider $W_1,\dotsc,W_5 \sim \mathcal{U}[0,1]$ and the regularization parameters are given by $\lambda_{n_1}^{\mu}=0.2 , \lambda_{n_2}^{\mu}=0.1, \lambda_{n_1}^{\sigma}=2.1$ and $\lambda_{n_2}^{\sigma}=1.0$. Here the parameters for the variance estimation are chosen so that we obtain the highest possible probability for sign-consistency. However, these results are not comparable to the ones in the scenarios (a) and (b). The plots in Figure \ref{figure:6} suggest that the fourth variance and all non-zero covariances are set to zero in some iterations of the first simulation. In the second one problems persist only with the covariance $\Sigma_{13}^*$, and the empirical densities of the covariances $\Sigma_{12}^*, \Sigma_{24}^*$ and $\Sigma_{34}^*$ look much better. Apparently positive and negative values of the covariates are crucial for the variable selection of the second moments.
 
\begin{gather*}
	\mathbb{P}\Big( \sign\big(\widehat{\mu}_{n_1}^{\,\AL}\big) = \sign\big(\mu^*\big)\Big) = 0.861\,,\qquad \mathbb{P}\Big( \sign\big(\widehat{\mu}_{n_2}^{\,\AL}\big) = \sign\big(\mu^*\big)\Big) = 0.917 \,,\\
	\mathbb{P}\Big( \sign\big(\widehat{\sigma}_{n_1}^{\,\AL}\big) = \sign\big(\sigma^*\big)\Big) = 0.0021\,,\qquad \mathbb{P}\Big( \sign\big(\widehat{\sigma}_{n_2}^{\,\AL}\big) = \sign\big(\sigma^*\big)\Big) = 0.1024\,.
\end{gather*}

\begin{figure}[h!]       
	\centering
	\includegraphics[width=0.85\linewidth]{mu_unif[0,1].eps}
	\caption{comparison of the densities of the rescaled estimation error of the means with $\mathcal{U}[0,1]$ distributed covariates.}
\end{figure}

\hfill
\newpage

\begin{figure}[h!]      
	\centering
	\includegraphics[width=0.85\linewidth]{sigma_unif[0,1].eps}
	\caption{comparison of the densities of the rescaled estimation error of the variances with $\mathcal{U}[0,1]$ distributed covariates.}
	\label{figure:6}
\end{figure}

\end{itemize}

==> structure_errors_second_moments.tex <==


\begin{remark}[Elastic net]% \label{remark:eps:sigma:first:moments:known} %\hfill\\
%
Mention the elastic net, theory extends, but numerical performance may be better, since covariates in the design matrix $\Xsigma$ may be highly correlated. 
%
\end{remark}

\begin{remark}[Asymptotic covariance matrix] \label{remark:cov:epsilon:second:moments} %\hfill\\
%
The asymptotic covariance matrix in \eqref{asymptotic:normality:adaptive:LASSO:second:moments} involves the matrix $\Psi^*$ and thus the matrices $\mathcal{M}^{kl}$ in \eqref{def:Mkl}. One can show that these are given more explicitely by 
	\begin{align*}
	\mathcal{M}^{kl} &= \mathcal{K}^{kl} - \kappa^{kl} \big(\mu^*\big)^\top - \mu^* \big( \kappa^{kl} \big)^\top  + \mu_l^* \Big(\kappa^k \big(\mu^*\big)^\top + \mu^* \big(\kappa^k\big)^\top - \mathcal{K}^{k} \Big)  \\
	& \quad \quad  \quad \quad + \mu_k^* \Big(\kappa^l \big(\mu^*\big)^\top +  \mu^* \big(\kappa^l\big)^\top - \mathcal{K}^{l} \Big)  \,.
\end{align*}
where 
%
% is symmetric and contains the (mixed) forth central moments of the coefficients $\f{A}$. Since we claimed in Lemma \ref{lemma:cov:epsilon:second:moments} the existence of the fourth moments, the Cauchy Schwarz inequality implies the well-definedness of $\mathcal{M}^{11},\mathcal{M}^{12}, $ $ \dotsc,\mathcal{M}^{pp}$ and especially $\Psi^*$. In addition note that the matrix $\mathcal{M}^{kl}$ is symmetric and that $\mathcal{M}^{kl}$ and $\mathcal{M}^{lk}$ are equal for $k,l \in \{1,\dotsc,p\}$. Hence no information about the fourth central moments has been lost in the definition of $\Psi^*$. Moreover, let	$\mathcal{K}^{kl},\mathcal{K}^{k} \in \R^{p \times p}$ and $\kappa^{kl},\kappa^{k} \in \R^{p}$ for $k,l \in \{1,\dotsc,p\}$ with
	\begin{align*}
		\big( \mathcal{K}^{kl} \big)_{uv} &\defeq \cov\big(A_{k} A_{l}, A_{u}A_{v} \big) \, , \qquad 
		\big( \mathcal{K}^{k} \big)_{uv} \defeq \cov\big(A_{k}, A_{u}A_{v} \big)  \, ,\\ 
		\big( \kappa^{kl} \big)_{u} &\defeq  \cov\big(A_{k} A_{l}, A_{u} \big) \, ,\qquad 
		\big( \kappa^{k} \big)_{u} \defeq  \cov\big(A_{k}, A_{u} \big) \,.
	\end{align*}
%
Using estimates of higher-order moments of the random coefficients, which can be obtained from linear regression equations similarly to those for the covariances, one can in principle construct a consistent estimator. 

{\color{red} Discuss, should not be used, mention post-selection inference theory}
%
\end{remark}
%\begin{remark} \label{remark:eps:sigma:first:moments:known} %\hfill\\
%	In the special case where the first moments $\mu^*$ of the coefficients are known in advance, we can set $\widehat{\mu}_n = \mu^*$.  As a consequence the matrices $E_n$ and $F_{1,n},\dotsc,F_{n,n}$ are equal to the null matrix and the linear regression model \eqref{random:coefficient:model:second:moments} simplifies to 
%	\begin{align*}
%		Y_i^{\sigma} = \ov\big(\f{X_i}\big)^\top \sigma^* +  \ov\big(\f{X_i}\big)^\top \ovec\big( D_i - \Sigma^* \big)\,, \quad i=1,\dotsc,n \,,
%	\end{align*}
%	respectively the error vector in \eqref{random:coefficient:model:second:moments:matrix} is $\epssigma = \delta_n$. In this case the heteroscedastic errors are independent as well.
%\end{remark}
%
In the following lemma we want to provide the conditional first and second moments of the error vector $\delta_n$, which is not influenced by the estimator error of the first moments. The proof is deferred to the supplement, Section \ref{sec:proof:lemma:cov:epsilon:second:moments}.



==> structure_model_first_moments.tex <==

 

To conduct statistical interference we observe independent and identically distributed pairs \linebreak $(Y_1,\f{W_1^\top})^\top,\dotsc,(Y_n,\f{W_n^\top})^\top$ of data according to the linear random coefficient regression model \eqref{random:coefficient:model:intercept}. We write
\begin{align}
Y_i =  B_{i,0} + \f{W_i^\top} \f{B_{i}} = \f{X_i^\top} \f{A_i} \,, \quad i =1,\dotsc,n\,,   \label{random:coefficient:model}
\end{align}
where $\f{X_i} = ( 1, \f{W_i^\top} )^\top \in \R^p$ with $\f{W_i} \sim \f{W}$ and $\f{A_i} = (B_{i,0},\f{B_{i}^\top} )^\top \sim \f{A}$ are independent random vectors. Here $\f{X_i} = ( X_{i,1},\dotsc,X_{i,p} )^\top$ represents the observed individual covariates and $\f{A_i} = ( A_{i,1},\dotsc,A_{i,p})^\top$ the unobserved independent and identically distributed, individual regression coefficients.\\

With the definition \eqref{def:mean:true} of the mean vector of the coefficients we can rewrite model \eqref{random:coefficient:model} by
\begin{align}
Y_i  = \f{X_i^\top} \mu^*  +  \f{X_i^\top} \big( \f{A_i} - \mu^* \big) \,, \quad i =1,\dotsc,n  \,, \label{random:coefficient:model:first:moments}
\end{align}
where the deterministic parameter vector $\mu^*$ is $s_\mu$-sparse and the errors are evidently heteroscedastic. We define         
\begin{align*}
\Ymu &\defeq \big( Y_1,\dotsc,Y_n \big)^\top  &&\in \R^n \, ,  \\
\Xmu &\defeq \big[ \f{X_1}, \dotsc, \f{X_n} \big]^\top  &&\in \R^{n \times p} \, , \\
\epsmu &\defeq \Big(  \f{X_1^\top} \big(\f{A_1} - \mu^*\big),\dotsc,\f{X_n^\top} \big(\f{A_n}-\mu^*\big) \Big)^\top &&\in \R^n
\end{align*}
and hence we can express \eqref{random:coefficient:model:first:moments} in matrix form by
\begin{align*}
\Ymu = \Xmu \, \mu^* + \epsmu = \XmuS \, \mu_{S_{\mu}}^* + \epsmu \,. %\label{random:coefficient:model:first:moments:sparse} 
\end{align*}
The entries of $\epsmu$ are pairwise independent and identically distributed since $(\f{X_1^\top}, \f{A_1^\top})^\top,$ \linebreak $\dotsc, (\f{X_n^\top}, \f{A_n^\top})^\top$ are independent and identically distributed. The conditional mean of $\epsmu$ regarding the covariates is given by
\begin{align}
\E\big[ \epsmu \,\big| \, \Xmu \big] = \Big(  \f{X_1^\top} \big(\E[\f{A_1}]-\mu^*\big),\dotsc,\f{X_n^\top} \big(\E[\f{A_n}]-\mu^* \big ) \Big)^\top  = \f{0}_n \label{mean:epsilon:first:moments}
\end{align} 
and the conditional variances of the entries of the error term satisfy
\begin{align*}
\var\Big( e_i^\top \epsmu \, \Big| \, \f{X_i} \Big) = \var\Big( \f{X_i^\top} \big( \f{A_i} - \mu^* \big) \, \Big| \, \f{X_i} \Big) = \sum_{k,l=1}^p   X_{i,k}  X_{i,l} \, \cov\big( A_{i,k}, A_{i,l} \big) = \f{X_i^\top} \Sigma^* \, \f{X_i} \,.
\end{align*}
Hence we obtain the conditional covariance matrix 
\begin{align}
\Omega_n^{\mu} \defeq \cov\big(\epsmu \, \big| \, \Xmu \big) = \diag \big( \f{X_1^\top} \Sigma^* \, \f{X_1} , \dotsc, \f{X_n^\top} \Sigma^* \, \f{X_n} \big) \, . \label{cov:epsilon:first:moments}
\end{align}


\begin{remark} \label{remark:cov:epsilon:positive:definite:first:moments} %\hfill\\
	The matrix $\Omega_n^{\mu} $ is obviously positive definite if the values $\f{X_1^\top} \Sigma^* \, \f{X_1} , \dotsc,$ \linebreak $\f{X_n^\top} \Sigma^* \, \f{X_n}$ are positive. That is generally given if the covariance matrix $\Sigma^*$ of the random coefficients $\f{A}$ is positive definite and $\f{X_1},\dotsc,\f{X_n} \neq  \f{0}_p$. However, we allow also sparsity of the second central moments of the coefficients, and therefore the covariance matrix can be positive semi-definite. Especially, as we mentioned before, if some of the coefficients are deterministic, the covariance matrix has rows and columns with zeros and in consequence no full rank. In that case the covariance matrix of the coefficients can be expressed by
	\begin{align*}
	\Sigma^* = \begin{bmatrix}   
	\Sigma_1^* & \f{0}_{d \times (p-d)}  \\
	\f{0}_{(p-d) \times d} & \f{0}_{(p-d) \times (p-d)} 
	\end{bmatrix}
	\end{align*}
	with $\Sigma_1^* \in \R^{d \times d}$, $d \leq p$ (change the order of the coefficients and the associated explanatory variables to get the block form). So if we assume $\Sigma_1^*$ to be positive definite and the corresponding covariates $(X_{1,1},\dotsc,X_{1,d})^\top, \dotsc, (X_{n,1},\dotsc,X_{n,d})^\top \neq \f{0}_d$, then the conditional covariance matrix $\Omega_n^{\mu} $ of the errors $\epsmu$ is still positive definite.
\end{remark}

Consider the linear regression model \eqref{random:coefficient:model:first:moments} of the first moments. The appropriate empirical quadratic loss function is defined by
\begin{align*}
	\loss_{\mu,n}^{\, \LS} \big(\beta\big) \defeq \frac{1}{n} \, \normzq{\Ymu - \X_n^{\mu} \, \beta} = \frac{1}{n} \sum_{i=1}^n \big( Y_i - \f{X_i^\top} \beta \big)^2 \,, \quad \beta \in \R^p \,. %\label{def:emprical:quadratic:loss:first:moments}
\end{align*} 
Then the adaptive LASSO with regularization parameter $\lambda_{n}^{\mu}$ is given by
\begin{align}
	\widehat{\mu}_n^{\,\AL} \in \rho_{\mu,n,\lambda_n^{\mu}}^{\,\AL} &\defeq \underset{\beta \in \R^p}{\arg\min} ~ \Bigg( \loss_{\mu,n}^{\, \LS} \big(\beta\big) +  2 \lambda_n^{\mu}  \sum_{k=1}^p \frac{|\beta_k|}{\big|\widehat{\mu}_{n,k}^{\,\init}\big|} \Bigg) \,, \label{def:adaptive:LASSO:first:moments}
\end{align}
where $\widehat{\mu}_n^{\,\init} \in \R^p$ is an initial estimator of $\mu^*$. If $\widehat{\mu}_{n,k}^{\,\init} = 0$, we require $\beta_k=0$, and, moreover, the sequence $\big(\widehat{\mu}_n^{\,\init}\big)_{n \in \N} \subset \R^p$ should be consistent with respect to $\mu^*$.  
